An Operational Framework for Nonclassicality in Quantum Communication Networks

Quantum resources, such as entanglement or quantum communication, offer significant communication advantages in information processing. We develop an operational framework for realizing these communication advantages in resource-constrained quantum networks. The framework computes linear bounds on the input/output probabilities of classical networks with limited communication and globally shared randomness. Since the violation of these classical bounds witnesses nonclassicality, a measurable communication advantage, the framework maximizes the violation of the classical bound using variational quantum optimization methods tailored to the communication network and quantum resources. This operational framework for nonclassicality can be scaled on quantum computers or deployed in the field to optimize noisy quantum networks for communication advantages. Applying this framework, we investigate the nonclassicality of communication networks that are assisted by quantum resources. We find that entanglement between communication-constrained parties is sufficient for nonclassicality to be found, whereas in networks with multiple senders, quantum communication with no entanglement-assistance is sufficient for nonclassicality to be found. As a result, entanglement is necessary for nonclassicality when a single sender broadcasts to multiple receivers.

==> tikz_figures/custom_commands.tex <==

% math commands
\newcommand{\mbf}{\mathbf}
\newcommand{\mbb}{\mathbb}
\newcommand{\mc}{\mathcal}
\newcommand{\N}{\mathcal{N}}
\newcommand{\tr}[1]{\textrm{Tr}\left[ #1 \right]}
\newcommand{\ptr}[2]{\textrm{Tr}_{#1} \left[ #2 \right]}
\newcommand{\id}{\textrm{id}}
% \newcommand{\ket}[1]{|#1\rangle}
% \newcommand{\bra}[1]{\langle #1|}
\newcommand{\ip}[1]{\langle#1\rangle}
\newcommand{\op}[2]{|#1\rangle\langle #2|}
\newcommand{\post}{\text{post}}
\newcommand{\1}{\mathds{1}}
\newcommand{\conv}[1]{\text{Conv}\left(#1\right)}
\newcommand{\cost}[1]{\text{Cost}\big(#1\big)}
\newcommand{\gain}[1]{\text{Gain}\big(#1\big)}
\newcommand{\Dim}[1]{\text{Dim}\left(#1\right)}

% notation commands
\newcommand{\Net}{\text{Net}}
\newcommand{\Dev}{\text{Dev}}
\newcommand{\Env}{\text{Env}}
\newcommand{\Rx}{\text{Rx}}
\newcommand{\Tx}{\text{Tx}}
\newcommand{\Mx}{\text{Mx}}
\newcommand{\Pbf}{\mbf{P}}
\newcommand{\PNet}{\Pbf^{\Net}}
\newcommand{\Gbf}{\mbf{G}}
\newcommand{\Vbf}{\mbf{V}}
\newcommand{\Fbf}{\mbf{F}}

\newcommand{\Amc}{\mc{A}}
\newcommand{\Bmc}{\mc{B}}
\newcommand{\Cmc}{\mc{C}}
\newcommand{\Emc}{\mc{E}}
\newcommand{\Hmc}{\mc{H}}
\newcommand{\Pbb}{\mbb{P}}
\newcommand{\Zbb}{\mbb{Z}}

\newcommand{\Bin}{\mbb{B}}
\newcommand{\Cbb}{\mbb{C}}
\newcommand{\Qbb}{\mbb{Q}}
\newcommand{\Vbb}{\mbb{V}}
\newcommand{\Fbb}{\mbb{F}}
\newcommand{\Xmc}{\mc{X}}
\newcommand{\Ymc}{\mc{Y}}
\newcommand{\Zmc}{\mc{Z}}
\newcommand{\Mmc}{\mc{M}}
\newcommand{\ANet}{\vec{\Amc}}
\newcommand{\BNet}{\vec{\Bmc}}
\newcommand{\CNet}{\vec{\Cmc}}
\newcommand{\MNet}{\vec{\Mmc}}
\newcommand{\XNet}{\vec{\Xmc}}
\newcommand{\YNet}{\vec{\Ymc}}
\newcommand{\ZNet}{\vec{\Zmc}}
\newcommand{\Av}{\vec{A}}
\newcommand{\Bv}{\vec{B}}
\newcommand{\Cv}{\vec{C}}
\newcommand{\Dv}{\vec{D}}
\newcommand{\Mv}{\vec{M}}
\newcommand{\Lambdav}{\vec{\Lambda}}
\newcommand{\Success}{\text{Success}}
\newcommand{\Error}{\text{Error}}


\newcommand{\av}{\vec{a}}
\newcommand{\bv}{\vec{b}}
\newcommand{\cv}{\vec{c}}
\newcommand{\dv}{\vec{d}}

\newcommand{\xv}{\vec{x}}
\newcommand{\yv}{\vec{y}}
\newcommand{\zv}{\vec{z}}
\newcommand{\reals}{\mbb{R}}
\newcommand{\Ibb}{\mbb{I}}

\newcommand{\EA}{\text{EA}}
\newcommand{\ERx}{\text{ERx}}
\newcommand{\ETx}{\text{ETx}}
\newcommand{\GEA}{\text{GEA}}
\newcommand{\GSR}{\text{GSR}}

\newcommand{\IF}{\text{IF}}
\newcommand{\CIF}{\text{CIF}}
\newcommand{\BF}{\text{BF}}
\newcommand{\HG}{\text{HG}}
\newcommand{\Post}{\text{Post}}
\newcommand{\XOR}{\text{XOR}}
\newcommand{\CV}{\text{CV}}
\newcommand{\ML}{\text{ML}}

% set notation
\newcommand{\set}[2]{\Big\{ #1 \;\Big|\; #2 \Big\}}

\newcommand{\PM}{\text{PM}}
\newcommand{\FF}{\text{FF}}
\newcommand{\BT}{\text{BS}}
% signaling scenarios
\newcommand{\XtoY}{\Xmc\text{\stackon[1pt]{$\to$}{$\scriptstyle d$}} \Ymc}
\newcommand{\XtoYtwo}{\Xmc\text{\stackon[1pt]{$\to$}{$\scriptstyle d$}} \Ymc_2}
\newcommand{\XtoYarb}[1]{\Xmc\text{\stackon[1pt]{$\to$}{$\scriptstyle #1$}} \Ymc}
\newcommand{\sigarb}[3]{#1 \text{\stackon[1pt]{$\to$}{$\scriptstyle #2$}} #3}
\newcommand{\CSigd}{\Cbb^{\XtoY}}
\newcommand{\CSigarb}[1]{\Cbb^{\XtoYarb{#1}}}

\newcommand{\QSigd}{\Qbb^{\XtoY}}


\newcommand{\BCgen}{\Xmc\text{\stackon[2pt]{$<$}{$\scriptstyle d$}}{\Ymc_1 \atop \Ymc_2}}
% \newcommand{\MAgen}{ {\Xmc_1 \atop \Xmc_2} \text{\stackon[2pt]{$>$}{$\scriptstyle d_1,d_2$}} \scriptstyle \Ymc}
\newcommand{\MAgen}{\text{MA}\left((\Xmc_i)_{i=1}^n,(d_i)_{i=1}^n,\Ymc\right)}
\newcommand{\MA}{\text{MA}}
\newcommand{\BC}{\text{BC}}
\newcommand{\precarb}[1]{\text{\stackon[2pt]{$<$}{$\scriptstyle #1$}}}

\newcommand{\Intgen}{ {\Xmc_1 \atop \Xmc_2} \text{\stackon[2pt]{$>$}{$\scriptstyle d$}} -  \text{\stackon[2pt]{$<$}{$\scriptstyle d$}} {\Ymc_1 \atop \Ymc_2}}

% color commands
\newcommand{\todo}[1]{{\color{red} #1}}

\theoremstyle{definition}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem*{example}{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem*{fact}{Fact}
\newtheorem{property}{Properties}
\newtheorem*{note}{Note}
\newtheorem*{remark}{Remark}
\newtheorem{claim}{Claim}
\newtheorem*{excercise}{Exercise}
\newtheorem{algorithm}{Algorithm}
\newtheorem{protocol}{Protocol}

\definecolor{prep_green}{HTML}{669933}
\definecolor{proc_red}{HTML}{CC3333}
\definecolor{meas_blue}{HTML}{3366CC}
\definecolor{quantum_purple}{HTML}{663366}
\definecolor{classical_gray}{HTML}{666666}



\usetikzlibrary{shapes,decorations,arrows,calc,arrows.meta,fit,positioning,external}
\tikzset{
    % auto,
    % -Latex,auto,node distance =1 cm and 1 cm,semithick,
    terminal/.style={},
    source/.style ={ellipse, draw, minimum width = 0.5 cm, color=classical_gray, fill=classical_gray!10, text=black},
    qsource/.style ={ellipse, draw, minimum width = 0.5 cm, color=prep_green, fill=prep_green!20, text=black},
    dev/.style={rectangle, rounded corners, draw, minimum width = 0.7 cm, color=classical_gray, fill=classical_gray!10, text=black},
    prep_dev/.style={dev, color=prep_green, fill=prep_green!20, text=black},
    proc_dev/.style={dev, color=proc_red, fill=proc_red!20, text=black},
    meas_dev/.style={dev, color=meas_blue, fill=meas_blue!20, text=black},
    el/.style = {align=left},
    meas_gate/.style={color=meas_blue, fill=meas_blue!20},
    prep_gate/.style={color=prep_green, fill=prep_green!20},
    proc_gate/.style={color=proc_red, fill=proc_red!20},
    arb_gate/.style={color=quantum_purple, fill=quantum_purple!20},
    classical_gate/.style={color=classical_gray, fill=classical_gray!20},
    meas_gate_group/.style={dashed,rounded corners,color=meas_blue},
    proc_gate_group/.style={dashed,rounded corners,color=proc_red},
    prep_gate_group/.style={dashed,rounded corners,color=prep_green},
}

\newcommand{\cedge}{edge[double, line width=1pt, double distance=1.5pt, arrows = {-Latex[length=0.5pt 2.5 0]}]}
\newcommand{\qedge}{edge[line width=2pt, arrows = {-Latex[length=6pt 1.5 0]}]}

==> tikz_figures/earx_quantum_broadcast_nonclassical_ansatz.tex <==
\begin{figure*}
    \centering
    \begin{tikzcd}[column sep=0.5cm]
            \gategroup[3,style={prep_gate_group, inner xsep=22pt, inner ysep=12pt, xshift=32pt}, label style={yshift=2pt}]{Source $\Lambda$} 
            \gategroup[2,style={meas_gate_group, inner xsep=92pt, inner ysep=12pt, xshift=219pt}, label style={yshift=2pt}]{Receiver $B_1$} 
            \lstick{$\ket{0}$} & \gate[style={prep_gate}]{H} & \ctrl{2}  & \qw & \ctrl{1} & \gate[style=meas_gate]{R_y(\vec{\theta}^{B_1}_{0})} & \ctrl{1} & \gate[style=meas_gate]{R_y(\vec{\theta}^{B_1}_{2})} & \meter[style={meas_gate}]{} & \rstick[2]{$y^{B_1}$}\cw \\
            \gategroup[3,style={prep_gate_group, inner xsep=25pt, inner ysep=12pt, xshift=90pt}, label style={yshift=-112pt}]{Sender $A$} 
            \lstick{$\ket{0}$} & \qw & \qw & \gate[style=prep_gate]{R_y(\vec{\theta}^A_{x,0})} & \targ{} & \gate[style=meas_gate]{R_y(\vec{\theta}^{B_1}_{1})} & \targ{} & \gate[style=meas_gate]{R_y(\vec{\theta}^{B_1}_{3})} & \meter[style={meas_gate}]{} & \cw \\ 
            \gategroup[2,style={meas_gate_group, inner xsep=92pt, inner ysep=12pt, xshift=219pt}, label style={yshift=-80pt}]{Receiver $B_2$} 
            \lstick{$\ket{0}$} & \qw & \targ{} & \qw & \ctrl{1} & \gate[style=meas_gate]{R_y(\vec{\theta}^{B_2}_{0})} & \ctrl{1} & \gate[style=meas_gate]{R_y(\vec{\theta}^{B_2}_{2})} & \meter[style={meas_gate}]{} & \rstick[2]{$y^{B_2}$}\cw \\
            \lstick{$\ket{0}$} & \qw & \qw  &  \gate[style=prep_gate]{R_y(\vec{\theta}^A_{x,1})} & \targ{} & \gate[style=meas_gate]{R_y(\vec{\theta}^{B_2}_{1})} & \targ{} & \gate[style=meas_gate]{R_y(\vec{\theta}^{B_2}_{3})} & \meter[style={meas_gate}]{} & \cw \\
        \end{tikzcd}
    \caption{Minimal variational ansatz circuit fpr entanglement-assisted receivers that achieves the maximal nonclassicality score. All rotations are about the $y$-axis on Bloch sphere such that $R_y(\vec{\theta}) = e^{-i \vec{\theta} \sigma_y/2}$. Note that the source $\Lambda$ operates upon the first and third qubits whereas the sender $A$ operates on the second and fourth qubits. The receivers each get one qubit from the sender and one qubit from the source. Furthermore, note that the sender does not prepare an entangled state. }
    \label{fig:earx_quantum_broadcast_nonclassicality_ansatz}
\end{figure*}
